Clustering Unclustered Data: Unsupervised Binary Labeling of Two Datasets Having Different Class Balances

We consider the unsupervised learning problem of assigning labels to unlabeled data. A naive approach is to use clustering methods, but this works well only when data is properly clustered and each cluster corresponds to an underlying class. In this paper, we first show that this unsupervised labeling problem in balanced binary cases can be solved if two unlabeled datasets having different class balances are available. More specifically, estimation of the sign of the difference between probability densities of two unlabeled datasets gives the solution. We then introduce a new method to directly estimate the sign of the density difference without density estimation. Finally, we demonstrate the usefulness of the proposed method against several clustering methods on various toy problems and real-world datasets.

==> New-Table-Paper-Np-40-Nq-40-theta-0.2-phi-0.8.tex <==


% 
% This table was automatically generated by code
%
% Np 40 Nq 40
% Theta 0.2 Phi 0.8
\begin{tabular}{p{1.55cm}p{1.7cm}p{1.7cm}p{1.7cm}p{1.7cm}p{1.7cm}l}
\toprule 
 \textbf{Dataset}& \textbf{DSDD}  & \textbf{LSDD}  & \textbf{KDE}  & \textbf{KM}  & \textbf{SC}  & \textbf{SMIC}   \\
 \midrule 
% Row 1 Dataset australian
australian & \textbf{.142} (.045)  & {.174} (.110)  & {.211} (.126)  & {.266} (.147)  & {.381} (.033)  & {.303} (.103) \\ 
 	 % 1558
% Row 2 Dataset banana
banana & {.179} (.097)  & \textbf{.170} (.070)  & {.237} (.147)  & {.431} (.068)  & {.427} (.141)  & {.424} (.141) \\ 
 	 % 1558
% Row 3 Dataset diabetes
diabetes & {.246} (.122)  & \textbf{.223} (.079)  & \textbf{.226} (.051)  & {.372} (.080)  & {.380} (.094)  & {.370} (.131) \\ 
 	 % 1577
% Row 4 Dataset german
german & {.268} (.059)  & {.281} (.127)  & \textbf{.211} (.051)  & {.437} (.114)  & {.448} (.128)  & {.439} (.052) \\ 
 	 % 1558
% Row 5 Dataset heart
heart & \textbf{.176} (.051)  & \textbf{.174} (.047)  & {.211} (.074)  & {.261} (.131)  & {.310} (.032)  & {.327} (.107) \\ 
 	 % 1558
% Row 6 Dataset image
image & \textbf{.198} (.078)  & {.206} (.047)  & \textbf{.201} (.049)  & {.385} (.093)  & {.351} (.119)  & {.384} (.135) \\ 
 	 % 1539
% Row 7 Dataset ionosphere
ionosphere & \textbf{.157} (.059)  & {.184} (.106)  & {.194} (.123)  & {.329} (.145)  & {.319} (.113)  & {.311} (.174) \\ 
 	 % 1558
% Row 8 Dataset saheart
saheart & {.310} (.093)  & \textbf{.205} (.048)  & {.238} (.113)  & {.422} (.121)  & {.395} (.113)  & {.384} (.072) \\ 
 	 % 1558
% Row 9 Dataset thyroid
thyroid & \textbf{.102} (.052)  & {.121} (.116)  & {.207} (.074)  & {.328} (.113)  & {.326} (.109)  & {.305} (.074) \\ 
 	 % 1558
% Row 10 Dataset twonorm
twonorm & {.044} (.085)  & {.051} (.072)  & {.200} (.028)  & \textbf{.036} (.054)  & {.043} (.069)  & {.048} (.071) \\ 
 	 % 1558
 
 \bottomrule \end{tabular}



==> New-Table-Paper-Np-40-Nq-40-theta-0.35-phi-0.65.tex <==


% 
% This table was automatically generated by code
%
% Np 40 Nq 40
% Theta 0.35 Phi 0.65
\begin{tabular}{p{1.55cm}p{1.7cm}p{1.7cm}p{1.7cm}p{1.7cm}p{1.7cm}l}
\toprule 
 \textbf{Dataset}& \textbf{DSDD}  & \textbf{LSDD}  & \textbf{KDE}  & \textbf{KM}  & \textbf{SC}  & \textbf{SMIC}   \\
 \midrule 
% Row 1 Dataset australian
australian & \textbf{.244} (.116)  & {.259} (.088)  & {.355} (.104)  & {.265} (.080)  & {.376} (.065)  & {.308} (.107) \\ 
 	 % 1577
% Row 2 Dataset banana
banana & \textbf{.338} (.094)  & \textbf{.339} (.100)  & {.365} (.067)  & {.433} (.049)  & {.427} (.069)  & {.424} (.070) \\ 
 	 % 1558
% Row 3 Dataset diabetes
diabetes & \textbf{.340} (.075)  & {.361} (.124)  & {.345} (.034)  & {.373} (.063)  & {.380} (.048)  & {.371} (.114) \\ 
 	 % 1558
% Row 4 Dataset german
german & {.375} (.042)  & {.380} (.093)  & \textbf{.354} (.057)  & {.437} (.024)  & {.445} (.057)  & {.438} (.041) \\ 
 	 % 1558
% Row 5 Dataset heart
heart & {.270} (.133)  & \textbf{.247} (.084)  & {.354} (.052)  & {.264} (.059)  & {.315} (.081)  & {.327} (.089) \\ 
 	 % 1558
% Row 6 Dataset image
image & \textbf{.331} (.078)  & {.350} (.067)  & {.350} (.039)  & {.384} (.031)  & {.354} (.049)  & {.382} (.050) \\ 
 	 % 1539
% Row 7 Dataset ionosphere
ionosphere & \textbf{.291} (.099)  & {.356} (.066)  & {.345} (.048)  & {.330} (.070)  & {.322} (.058)  & {.314} (.107) \\ 
 	 % 1539
% Row 8 Dataset saheart
saheart & {.378} (.093)  & \textbf{.353} (.057)  & {.363} (.066)  & {.419} (.082)  & {.395} (.022)  & {.385} (.040) \\ 
 	 % 1558
% Row 9 Dataset thyroid
thyroid & \textbf{.227} (.098)  & {.251} (.087)  & {.302} (.022)  & {.326} (.061)  & {.329} (.047)  & {.307} (.076) \\ 
 	 % 1520
% Row 10 Dataset twonorm
twonorm & {.164} (.188)  & {.153} (.121)  & {.352} (.096)  & \textbf{.036} (.053)  & {.042} (.122)  & {.049} (.120) \\ 
 	 % 1558
 
 \bottomrule \end{tabular}



==> OldOptimization.tex <==
\section{Optimization}
\label{sec:OptimizationAppendix}
The function in Eq.\eqref{eq:L1ObjectiveFunction} should satisfy the constraint $\left|g(\boldx) \right| \leq 1, \:\: \forall \boldx$. We can consider a clipped version of the function that always satisfies the constraint, 
\begin{align*}
\widetilde{g}(\boldx) = R(g(\boldx)),
\end{align*}
where
\begin{align*}
R(z) = \begin{cases}
1 & z > 1, \\
-1 & z < -1, \\
z & \mathrm{otherwise}.
\end{cases}
\end{align*}
We use a linear in parameter model, 
\begin{align*}
g(\boldx) = \sum_{\ell = 1}^b {\alpha_\ell \varphi_\ell(\boldx)},
\end{align*}
where $\varphi_\ell(\boldx)$ are the basis functions. We replace the integrals by their empirical averages and recast the objective function as a minimization problem. This gives the objective function to be minimized as
\begin{align}
J(\boldalpha) =  \frac{1}{n'}\sum_{i=1}^{n'}{R\left(\sum_{\ell=1}^b{\alpha_\ell \varphi_\ell(\boldx_i')}\right)} - \frac{1}{n}\sum_{j=1}^{n}{R\left(\sum_{\ell=1}^b{\alpha_\ell \varphi_\ell(\boldx_j)}\right)} + \frac{\lambda}{2}\sum_{\ell=1}^b{\alpha_i^2},
\label{eq:ObjectiveFunction}
\end{align}
where $\frac{\lambda}{2}\sum_{\ell=1}^b{\alpha_i^2}$ is a regularization term.

The above optimization problem is a non-convex problem. We can efficiently find a locally optimal solution using the convex-concave procedure \cite{Yuille02theconcave-convex} (also known as difference of convex programming \cite{horst1999dc}).
The essence of the CCCP procedure is that we calculate an upper-bound for the objective 
function by bounding the concave part. 
We then minimize the objective function by alternately minimizing the upper bound and then 
tightening the upper bound around a point. Both the minimization of the upper bound and the
tightening of the upper bound are convex problems.

The non-convex function $R(z)$ can be written as a convex and concave term, 
\begin{align*}
R(z) = C_{-1}(z) - C_{1}(z)-1,
\end{align*} 
where $C_{\epsilon}(z)$ is defined as 
\begin{align*}
C_{\epsilon}(z) = \max(0, z-\epsilon).
\end{align*}
The objective function can therefore be written as
\begin{align*}
J(\boldalpha) & = J_{\mathrm{vex}}(\boldalpha) + J_{\mathrm{cave}}(\boldalpha),
\end{align*}
where
\begin{align*}
J_{\mathrm{vex}}(\boldalpha) & = \frac{1}{n'}\sum_{i=1}^{n'}C_{-1}\left(\sum_{\ell=1}^{b}\alpha_\ell \varphi_\ell(\boldx_i') \right) + \frac{1}{n}\sum_{j=1}^nC_{1}\left(\sum_{\ell=1}^b \alpha_\ell (\boldx_j)  \right) + \frac{\lambda}{2}\sum_{\ell=1}^b{\alpha_i^2},
\end{align*}
and
\begin{align*}
J_{\mathrm{cave}}(\boldalpha) & = -\frac{1}{n'}\sum_{i=1}^{n'}C_{1}\left(\sum_{\ell=1}^b \alpha_\ell \varphi_\ell (\boldx_i') \right) - \frac{1}{n}\sum_{j=1}^n {C_{-1}\left(\sum_{\ell=1}^b \alpha_\ell \varphi_\ell (\boldx_j) \right)}.
\end{align*}
The following self-evident relation can be used to bound the concave part
\begin{align*}
tz - \varphi(t) & \leq \sup_{y\in \mathbbR} yz - \varphi(y) \\
\Rightarrow \varphi(t) & \geq tz - \varphi^\ast(z),
%\label{eq:LFBound}
\end{align*}
where 
\begin{align*}
\varphi^\ast(z) = \sup_{y\in \mathbbR} yz - \varphi(y)
\end{align*}
is known as the \emph{convex conjugate}. The convex conjugate of the 
function $C_\epsilon(z)$ is
\begin{align*}
C_\epsilon^\ast(z) = \begin{cases}
\infty & z < 0 \\
\epsilon z & 0 \leq z \leq 1 \\
\infty & z > 0.
\end{cases}
\end{align*}
This gives a bound of
\begin{align*}
\bar{J}_{\mathrm{cave}}(\boldalpha, \boldb, \boldc) & =  
% first term
\frac{1}{n'}\sum_{i=1}^{n'}{\left(C_{1}^\ast(b_i) - b_i\sum_{\ell=1}^b \alpha_\ell \varphi_\ell(\boldx_i')\right)} 
% second term 
+ \frac{1}{n}\sum_{j=1}^n{\left(C_{-1}^\ast(c_j) - c_j\sum_{\ell=1}^b \alpha_\ell \varphi_\ell(\boldx_j) \right)},
\end{align*}
where $\boldb = \left[b_1 \: b_2 \: \ldots \: b_{n'} \right]$ and $\boldc = \left[c_1 \: c_2 \: \ldots \: c_{n'} \right]$ specify the bound.
%
We can then express the objective function as
\begin{align}
\min_{\boldalpha} J(\boldalpha) \leq \min_{\boldalpha} \min_{\boldb,\boldc} J_{\mathrm{vex}}(\boldalpha) + \bar{J}_{\textrm{cave}}(\boldalpha, \boldb, \boldc).
\label{eq:UpperBoundMin}
\end{align}
We can therefore alternately minimize the upper bound w.r.t. $\boldalpha$ (assuming $\boldb$ and $\boldc$ is constant) and tighten the bound by minimizing w.r.t. $\boldb$ and $\boldc$ (assuming $\boldalpha$ is constant). 

\subsubsection{Tightening the bound}
We can tighten the bound by minimizing $J_{\textrm{cave}}(\boldb, \boldc)$, assuming $\boldalpha$ is constant. 
To ensure that the bound is non-trivial, we explicitly write the constraints
\begin{align*}
\begin{array}{cl}
\displaystyle \bar{J}_{\mathrm{cave}}(\boldalpha, \boldb, \boldc) & = \displaystyle \frac{1}{n'}\sum_{i=1}^{n'}{b_i \left(1- \sum_{\ell=1}^b \alpha_\ell \varphi_\ell(\boldx_i') \right) }
+ \frac{1}{n}\sum_{j=1}^n c_j\left(-1 - \sum_{\ell=1}^b \alpha_\ell \varphi_\ell(\boldx_j) \right) \\ 
% line 2 
& \phantom{=} \mathrm{s.t. } \:\: 0 \leq b_i \leq 1, 0 \leq c_i \leq 1.
\end{array}
\end{align*}
The above optimization problem is separable in all the unknowns. Therefore the optimal values are
\begin{align*}
b_i = \begin{cases}
0 & \sum_{\ell = 1}^b \alpha_\ell \varphi_\ell(\boldx_i') < 1, \\
1 & \mathrm{otherwise.}
\end{cases}
\end{align*}
The same can be done for $c_i$,
\begin{align*}
c_j = \begin{cases}
0 & \sum_{\ell=1}^b{\alpha_\ell \varphi(\boldx_j)} < -1, \\
1 & \mathrm{otherwise.}
\end{cases} 
\end{align*}

\subsubsection{Minimizing the upper bound}
By assuming that $\boldb$ and $\boldc$ are constant, the upper bound to be minimized is
%Assuming $\boldb$ and $\boldc$ is constant, the upper bound can be expressed as
\begin{align*}
\bar{J}(\boldalpha) & =  \frac{1}{n'}\sum_{i=1}^{n'}C_{-1}\left(\sum_{\ell=1}^{b}\alpha_\ell \varphi_\ell(\boldx_i') \right) + \frac{1}{n}\sum_{j=1}^n C_{1}\left(\sum_{\ell=1}^b \alpha_\ell \varphi_\ell(\boldx_j)  \right) \\
% bound, assuming b and c is constant
& \qquad - {\sum_{\ell = 1}^b{\alpha_\ell \frac{1}{n'} \sum_{i=1}^{n'} b_i \varphi_\ell(\boldx_i')}} - \sum_{\ell=1}^b \alpha_\ell \frac{1}{n}\sum_{j=1}^n c_j \varphi_\ell(\boldx_j) + \frac{\lambda}{2}\sum_{\ell=1}^b{\alpha_\ell^2}. 
\end{align*} 

To obtain an objective function that we can use in an off-the-shelf convex optimizer, 
we can rewrite the non-differentiable loss function as constraints. We replace each 
function $C_\epsilon(z)$ with a slack variable $\xi_i$, where we add the constraint
\begin{align*}
\xi_i \geq 0, \: \xi_i \geq z - \epsilon. 
\end{align*}
The upper bound can then be written as
\begin{align}
\begin{array}{cc}
%\bar{J}(\boldalpha) & = \frac{1}{n'}\sum_{i=1}^{n'}{\xi_i' } + \frac{1}{n}\sum_{j=1}^n{\xi_j} - \sum_{\ell=1}^b \alpha_\ell\frac{1}{n'} \sum_{i=1}^{n'}{b_i\varphi_\ell(\boldx_i')} - \sum_{\ell=1}^b \alpha_\ell \frac{1}{n}\sum_{j=1}^n c_j \varphi_\ell(\boldx_j) + F(\boldalpha).  \\
% row 2 
\displaystyle \bar{J}(\boldalpha) & = \displaystyle \frac{1}{n'}\sum_{i=1}^{n'}{\xi_i' } + \frac{1}{n}\sum_{j=1}^n{\xi_j} + \sum_{\ell=1}^b\alpha_\ell\left(\frac{1}{n'} \sum_{i=1}^{n'}{b_i\varphi_\ell(\boldx_i')}  + \frac{1}{n}\sum_{j=1}^n c_j \varphi_\ell(\boldx_j) \right)   + \frac{\lambda}{2}\sum_{\ell=1}^b{\alpha_\ell^2}. \\
% row 3
& \displaystyle \mathrm{s.t.}\:  \xi_i' \geq 0, \: \xi_i' \geq \sum_{\ell=1}^b{\alpha_\ell \varphi_\ell(\boldx_i')} +1, \:\: \forall  i=1, \ldots, n' \nonumber \\
& \displaystyle \phantom{\mathrm{s.t.}}\: \xi_j \geq 0, \: \xi_j \geq \sum_{\ell=1}^b{\alpha_\ell \varphi_\ell(\boldx_j)} - 1, \:\: \forall  j=1, \ldots, n.
\end{array} \\
\label{eq:UpperBoundProblem}
\end{align}
The above is a constrained quadratic program which can be solved with off-the-shelf optimizer.
%When the regularizer is $F(\boldalpha ) = \frac{1}{2}\left\|\boldalpha \right\|_2^2$, the above problem is a quadratic problem. When the regularizer is chosen as $F(\boldalpha) = \left\|\boldalpha \right\|_1$, it is a linear programming problem.

\subsubsection{Summary}
The algorithm for calculating the sign of the density difference can be summarized as:
\begin{enumerate}
  \item \emph{Initialize the starting value:} $\boldalpha^1 = \argmin_{\boldalpha} J_{\mathrm{vex}}(\boldalpha)$ \\
  \item \emph{For $t=1, \ldots $: } 
  \begin{enumerate}
    \item \emph{Tighten the upper-bound:} \newline \noindent
    The variables for the bound can be calculated as: 
\begin{align*}
b_i = \begin{cases}
0 & \sum_{\ell = 1}^b \alpha_\ell \varphi_\ell(\boldx_i') < 1, \\
1 & \mathrm{otherwise},
\end{cases}
\end{align*}
and
\begin{align*}
c_j = \begin{cases}
0 & \sum_{\ell=1}^b{\alpha_\ell \varphi(\boldx_j)} < -1, \\
1 & \mathrm{otherwise.}
\end{cases} 
\end{align*}
	  \item \emph{Minimize the upper bound: } \newline \noindent
	  Determine
	  \begin{align*}
	  \boldalpha^{t+1} = \argmin_{\boldalpha} {\bar{J}(\boldalpha)},
	  \end{align*}
	  where this is by solving the convex problem in Eq.\eqref{eq:UpperBoundProblem}.
    \end{enumerate} 
\end{enumerate}
The above procedure is performed until $\left\|\boldalpha^{t+1} - \boldalpha^t \right\|_2 \leq E$, where $E$ determines the stopping criterion. 


==> fundamentalstrategyold.tex <==

\subsection{Fundamental Strategy}
Due to the class-balance change assumption in Eq.\eqref{eq:ClassPriorChangeAssumption},
we can express the two distributions from which $\calX_p$ and $\calX_{p'}$ are drawn as
\begin{align*}
\density(\boldx) &= \density(\boldx|y=1)\density(y=1) + \density(\boldx|y=-1)\density(y=-1), \\
\density'(\boldx) &= \density(\boldx|y=1)\density'(y=1) + \density(\boldx|y=-1)\density'(y=-1), 
\end{align*}
where the distributions differ only by a change in class balance.
Our central idea to obtain a labeling is 
to calculate the difference between the above two input densities:
% marginal densities
\begin{align*}
\density(\boldx) - \density'(\boldx) & = \density(y=1)\density(\boldx|y=1) +\left[1-\density(y=1) \right]\density(\boldx|y=-1) \\
& \phantom{=}
- \density'(y=1)\density(\boldx|y=1) - \left[1-\density'(y=1)\right]\density(\boldx|y=-1) \\
& = \left[\density(y=1) - \density'(y=1)\right]\left[\density(\boldx|y=1) - \density(\boldx|y=-1)  \right] \\
& \propto p(\boldx|y=1) - p(\boldx|y=-1).
\end{align*}
We can therefore obtain a label
by considering the sign of the term $\density(\boldx|y=1) - \density(\boldx|y=-1)$.
This corresponds to a classifier that assumes an equal class-balance.
%Thus the class label can be obtained from the term $\density(\boldx|y=1) - \density(\boldx|y=-1)$. 
Since the term $\density(y=1) - \density'(y=1)$ can be positive or negative, we can not recover the exact class label\footnote{If we know the class balance of the two datasets or know which class balance is larger, we can recover the exact label. We assume here the more general case where the class balance of both datasets is completely unknown.}. Therefore, we assign the label $y \in \left\{ 1,-1\right\}$ to a point $\boldx$ according to the following criterion:
\begin{align}
y = \operatorname{sign}{\left[\density(\boldx) - \density'(\boldx)  \right]}.
\label{eq:LabelingCriterion} 
\end{align}

Thus, now we need a good method to estimate
$\operatorname{sign}{\left[\density(\boldx) - \density'(\boldx)  \right]}$.

% \section{Review of the density difference estimation approach}
% In this section we discuss existing methods to estimate the density difference
% \begin{align*}
% \density(\boldx) - \density'(\boldx).
% \end{align*}
% If an estimator of the density difference is known, we can substitute it into Eq.~\eqref{eq:LabelingCriterion} to obtain a labeling. We briefly review two 
% methods for estimating the density difference: difference of kernel density estimators (KDEs) and direct estimation via least-squares fitting.

==> hingelosscomparison.tex <==
\section{Comparison with the Hinge loss}
We show here that by omitting a concave term, the objective function is similar to the Hinge loss. We further show with the aid of an example that while the omission of the concave term is
an acceptable assumption in the classification setting, it is not good for the class-balance change labeling setting where distributions overlap.  
The Hinge loss is defined as 
\begin{align*}
H_{\epsilon}(z) = \max(0, \epsilon - z).
\end{align*}
We can rewrite the function $R(z)$ in terms of the Hinge loss as
\begin{align*}
R(z) = H_1(-z) - H_{-1}(-z), \: \textrm{and} :\ R(z) = -H_{1}(z) + H_{-1}(z).
\end{align*}
Applying these relations to the objective function gives
\begin{align*}
\mathrm{minimize}  & \frac{1}{n'}\sum_{j=1}^{n'}{H_1(-g(\boldx_j'))} + \frac{1}{n'}\sum_{j=1}^{n'}{ H_{-1}(-g(\boldx_j'))} \\
 & -\frac{1}{n}H_{1}(g(\boldx_i)) + \frac{1}{n}\sum_{i=1}^{n}{H_{-1}(g(\boldx_i))}
\end{align*}
The above problem is non-convex, but we can relax it by ignoring all the concave terms. This
gives
\begin{align*}
\mathrm{minimize}  & \frac{1}{n'}\sum_{j=1}^{n'}{H_1(-g(\boldx_j'))} + \frac{1}{n}\sum_{i=1}^{n}{H_{-1}(g(\boldx_i))}.
\end{align*}
The objective function of the SVM can be written in terms of a Hinge loss function (where we omitted the regularization term)
\begin{align}
\sum_{i=1}^{N}H_{1}(y_i g(\boldx_i)),
\label{eq:SVMHingeLoss}
\end{align}
where the labeled samples are denoted as $\left\{\boldx_i, y_i \right\}_{i=1}^N$ and $y\in\left\{ -1, 1\right\}$.
Comparing the objective function with that of SVM (assuming an equal number of samples 
between the classes), we see that it is identical. We show in Section~\ref{sec:FailureOfHingeLoss}, with 
the aid of an example, that the assumption of ignoring the concave term is 
reasonable for classification problems when the classes do not significantly overlap. 
But for our problem, the overlapping of densities causes a big problem. 



\subsection{Numerical Illustration: Failure of the Hinge loss}
\label{sec:FailureOfHingeLoss}
We illustrate the failure of the Hinge loss by comparing the following to objective functions:
\begin{align*}
J(\boldw) = \frac{1}{n}\sum_{i=1}^n{H_{-1}(\boldw^\top\boldx + b )} + \frac{1}{n'}\sum_{j=1}^{n'}H_{1}\left(-\boldw^\top \boldx + b\right) + \frac{\lambda}{2}\boldw^\top \boldw,  
\end{align*}
and
\begin{align*}
J(\boldw) = \frac{1}{n}\sum_{i=1}^n{R(\boldw^\top + b )} - \frac{1}{n'}\sum_{j=1}^{n'}R\left(\boldw^\top\boldx + b\right) + \frac{\lambda}{2}\boldw^\top \boldw.
\end{align*}
We set $\lambda = 1^{-3}$. The second coordinate has the same normal distribution for both 
classes. The second coordinate is distributed uniformly from $0$ to $5$ for the red class.
For the black class, the coordinate is uniformly distributed from $5$ to $10$ in Figure~\ref{fig:Toy4a} and from $0$ to $10$ in Figure~\ref{fig:Toy4b}.  
\begin{figure}
        \centering
        \begin{subfigure}[b]{0.4\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/toy4ex1} 
               \caption{Non-overlapping distributions}
                \label{fig:Toy4a}
        \end{subfigure}
        \begin{subfigure}[b]{0.4\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/toy4ex2}
                \caption{Overlapping distributions.}
                \label{fig:Toy4b}
        \end{subfigure}
        \caption{Illustration of the failure of the Hinge loss in overlapping data.}
        \label{fig:HingeLossFailure}        
\end{figure}
When the classes are separable, the solution to the SVM and our method coincides. 
When the classes are overlapping, the solution of SVM differs significantly from our 
method and the optimal method. This is due to the rejection of the concave part of the 
objective function (which corresponds to the assumption that the classes do not overlap).

Due to the fact that class balance change occurs, datasets where the distributions overlap will
occur frequently in our problem. Therefore the default SVM solution will not perform well.


==> illus1.tex <==
\begin{picture}(0,0)%
\includegraphics{images/illus1}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2{%
  \fontsize{#1}{#2pt}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4740,3495)(1655,-3601)
%  METADATA <id>2</id> 
\put(5198,-1287){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\color[rgb]{0,0,0}$p(\boldx|y=1)$}%
}}}}
%  METADATA <id>3</id> 
\put(3544,-2468){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\color[rgb]{0,0,0}$p(\boldx|y=-1)$}%
}}}}
\end{picture}%





==> oldtables.tex <==
\begin{table}
\centering
\small
\caption{Labeling error rate for experiments with a class prior of $p(y=1)=0.2$ and $p'(y=1)=0.8$. The size of each dataset was $\left| \calX_{p}\right| = 40$ and $\left| \calX_{p'}\right| = 40$. The best method in terms of the mean error and
comparable methods according to the two-sided paired t-test at the significance level 5\%
are specified by bold face. The standard deviation of the labeling error rate is given in brackets.}
\input{New-Table-Paper-Np-40-Nq-40-theta-0.2-phi-0.8.tex}
%\caption{$N=30 \: 0.3 \: 0.6$}
\label{tab:Results-02-08}
\end{table}
%
% 
%
\begin{table}
\centering
\small
\caption{Labeling error rate for experiments with a class prior of $p(y=1)=0.35$ and $p'(y=1)=0.65$. The size of each dataset was $\left| \calX_{p}\right| = 40$ and $\left| \calX_{p'}\right| = 40$. The best method in terms of the mean error and
comparable methods according to the two-sided paired t-test at the significance level 5\%
are specified by bold face. The standard deviation of the labeling error rate is given in brackets.}
\input{New-Table-Paper-Np-40-Nq-40-theta-0.35-phi-0.65.tex}
%\caption{$N=30 \: 0.3 \: 0.6$}
\label{tab:Results-035-065}
\end{table}

==> toyprob1.tex <==
\subsubsection{Toy Problem 1:}
We illustrate the problem and our method with a simple example. Suppose that the class-conditional densities for the two classes are given as 
\begin{align*}
p(\boldx|y=1) = \calN_\boldx\left(-\bold1_{2}, \boldI_{2\times 2}\right) 
~~\mbox{and}~~
p(\boldx|y=-1) = \calN_\boldx\left(\bold1_{2}, \boldI_{2\times 2}\right),
\end{align*}
where $\calN_\boldx(\boldmu,\boldSigma)$ denotes the normal density
with mean $\boldmu$ and covariance $\boldSigma$ w.r.t. $\boldx$.
$\bold1_{2}$ is a $2\times 1$ vector of ones and $\boldI$ is a $2\times 2$ identity matrix. We generate $2$ sets of $30$ samples
with class-priors $p(y=1)=0.3$ and $p'(y=1)=0.6$, respectively.
%  from each class according to the following class priors: 
% \begin{align*}
% \theta = 0.3, \qquad \phi = 0.6.
% \end{align*} 
The result is illustrated in Figure~\ref{fig:toyillustration}. As can be seen from this example, we are able to obtain a labeling of the classes that roughly corresponds to the true (unknown) labels of the data.
%\usepackage{graphics} is needed for \includegraphics

\begin{figure}[t]
        \centering
        \begin{subfigure}[b]{0.325\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/toynew} 
               \caption{}
                \label{fig:originalData}
        \end{subfigure}%
        \begin{subfigure}[b]{0.325\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/toyexample3}
                \caption{}
                \label{fig:labellingXp} 
        \end{subfigure}
        \begin{subfigure}[b]{0.325\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/toyexample4}
                \caption{}
                \label{fig:labellingXq} 
        \end{subfigure}
        \caption{Illustrative example of the class-prior change labeling method. Figure~\ref{fig:originalData} shows the samples of datasets $\calX_p$ and $\calX_{p'}$, drawn from $p(\boldx)$ and $p'(\boldx)$. Figures~\ref{fig:labellingXp} and \ref{fig:labellingXq} illustrate the discriminant applied to the datasets $\calX_{p}$ and $\calX_{p'}$. The estimated discriminant is given in blue and the optimal discriminant is in black. The true underlying class labels (which are unknown) are illustrated in red and black.  }\label{fig:toyillustration}
\end{figure}

